Privileged Attribution Constrained Deep Networks for Facial Expression Recognition

Facial Expression Recognition (FER) is crucial in many research domains because it enables machines to better understand human behaviours. FER methods face the problems of relatively small datasets and noisy data that don't allow classical networks to generalize well. To alleviate these issues, we guide the model to concentrate on specific facial areas like the eyes, the mouth or the eyebrows, which we argue are decisive to recognise facial expressions. We propose the Privileged Attribution Loss (PAL), a method that directs the attention of the model towards the most salient facial regions by encouraging its attribution maps to correspond to a heatmap formed by facial landmarks. Furthermore, we introduce several channel strategies that allow the model to have more degrees of freedom. The proposed method is independent of the backbone architecture and doesn't need additional semantic information at test time. Finally, experimental results show that the proposed PAL method outperforms current state-of-the-art methods on both RAF-DB and AffectNet.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************


==> images/figures/half_maps.tex <==
\begin{figure*}[!t]
\centering
\subfloat{\includegraphics[width=0.825in]{images/half_maps2/0301_first.jpg}%
\label{ha1}}
\hfil
\subfloat{\includegraphics[width=0.825in]{images/half_maps2/0212_first.jpg}%
\label{ha2}}
\hfil
\subfloat{\includegraphics[width=0.825in]{images/half_maps2/0524_first.jpg}%
\label{ha3}}
\hfil
\subfloat{\includegraphics[width=0.825in]{images/half_maps2/0116_first.jpg}%
\label{ha4}}
\hfil
\subfloat{\includegraphics[width=0.825in]{images/half_maps2/0125_first.jpg}%
\label{ha5}}
\hfil
\subfloat{\includegraphics[width=0.825in]{images/half_maps2/0134_first.jpg}%
\label{ha6}}
\hfil
\subfloat{\includegraphics[width=0.825in]{images/half_maps2/0214_first.jpg}%
\label{ha7}}
\hfil
\subfloat{\includegraphics[width=0.825in]{images/half_maps2/0008_first.jpg}%
\label{ha8}}
\hfil
\vfil
\subfloat{\includegraphics[width=0.825in]{images/half_maps2/0301_second.jpg}%
\label{hf1}}
\hfil
\subfloat{\includegraphics[width=0.825in]{images/half_maps2/0212_second.jpg}%
\label{hf2}}
\hfil
\subfloat{\includegraphics[width=0.825in]{images/half_maps2/0524_second.jpg}%
\label{hf3}}
\hfil
\subfloat{\includegraphics[width=0.825in]{images/half_maps2/0116_second.jpg}%
\label{hf4}}
\hfil
\subfloat{\includegraphics[width=0.825in]{images/half_maps2/0125_second.jpg}%
\label{hf5}}
\hfil
\subfloat{\includegraphics[width=0.825in]{images/half_maps2/0134_second.jpg}%
\label{hf6}}
\hfil
\subfloat{\includegraphics[width=0.825in]{images/half_maps2/0214_second.jpg}%
\label{hf7}}
\hfil
\subfloat{\includegraphics[width=0.825in]{images/half_maps2/0008_second.jpg}%
\label{hf8}}
\hfil
\vfil
\subfloat{\includegraphics[width=0.825in]{images/half_maps2/0301_baseline.jpg}%
\label{hb1}}
\hfil
\subfloat{\includegraphics[width=0.825in]{images/half_maps2/0212_baseline.jpg}%
\label{hb2}}
\hfil
\subfloat{\includegraphics[width=0.825in]{images/half_maps2/0524_baseline.jpg}%
\label{hb3}}
\hfil
\subfloat{\includegraphics[width=0.825in]{images/half_maps2/0116_baseline.jpg}%
\label{hb4}}
\hfil
\subfloat{\includegraphics[width=0.825in]{images/half_maps2/0125_baseline.jpg}%
\label{hb5}}
\hfil
\subfloat{\includegraphics[width=0.825in]{images/half_maps2/0134_baseline.jpg}%
\label{hb6}}
\hfil
\subfloat{\includegraphics[width=0.825in]{images/half_maps2/0214_baseline.jpg}%
\label{hb7}}
\hfil
\subfloat{\includegraphics[width=0.825in]{images/half_maps2/0008_baseline.jpg}%
\label{hb8}}
\hfil
\caption{On the first and second rows, examples of \textit{Grad*Input} attribution maps for the PAL-trained model with \textit{Mean of Half} channel strategy. The first row shows the mean map for the first half of the channels (constrained) while the second row shows the mean map for the second half of the channels (not constrained). On the third row, \textit{Grad*Input} attribution maps without PAL. Examples are chosen from the RAF-DB test set.}
\label{half_maps}
\end{figure*}

==> images/figures/heatmaps_fig.tex <==
\begin{figure}[!t]
\centering
\subfloat{\includegraphics[width=1.1in]{images/activation maps/anger_surprise_baseline.jpg}%
\label{7}}
\hfil
\subfloat{\includegraphics[width=1.1in]{images/activation maps/surprise_fear_baseline.jpg}
\label{8}}
\subfloat{\includegraphics[width=1.1in]{images/activation maps/disg_ang_baseline.jpg}%
\label{9}}
\vfil
\subfloat{\includegraphics[width=1.1in]{images/activation maps/anger_surprise_heatmap.jpg}%
\label{10}}
\hfil
\subfloat{\includegraphics[width=1.1in]{images/activation maps/surprise_fear_heatmap.jpg}%
\label{11}}
\hfil
\subfloat{\includegraphics[width=1.1in]{images/activation maps/disg_ang_heatmap.jpg}%
\label{12}}
\caption{Examples of \textit{Grad} attribution maps with (bottom row) and without (top row) PSL on RAF-DB test samples.}
\label{attributions}
\end{figure}

==> images/figures/raf_imgs_table.tex <==
\begin{figure*}[!t]
\centering
\subfloat[Sadness (Fear)]{\includegraphics[width=1.1in]{images/labeled_raf_imgs/test_2270_aligned.jpg}%
\label{1}}
\hfil
\subfloat[Surprise (Fear)]{\includegraphics[width=1.1in]{images/labeled_raf_imgs/test_2297_aligned.jpg}%
\label{2}}
\hfil
\subfloat[Neutral (Disgust)]{\includegraphics[width=1.1in]{images/labeled_raf_imgs/test_2357_aligned.jpg}%
\label{3}}
\hfil
\subfloat[Anger (Disgust)]{\includegraphics[width=1.1in]{images/labeled_raf_imgs/test_2365_aligned.jpg}%
\label{4}}
\hfil
\subfloat[Anger (Anger)]{\includegraphics[width=1.1in]{images/labeled_raf_imgs/test_0017_aligned.jpg}%
\label{5}}
\hfil
\subfloat[Anger (Anger)]{\includegraphics[width=1.1in]{images/labeled_raf_imgs/test_0190_aligned.jpg}%
\label{6}}
\caption{Test samples with the predicted emotion and the ground-truth emotion in parenthesis}
\label{raf_examples}
\end{figure*}

==> sections/old_related.tex <==
We aim to spatially constrain our FER model by guiding its attribution maps. Thus, we will first present methods that spatially constrain their models for Facial Expression tasks, and we will then focus on methods that directly constrain their attributions.

\subsubsection{Constrained Attribution Learning}

Recent work has been done to improve the interpretablility of Deep Neural Networks \cite{ancona2018better}. Attribution methods, also sometimes called "relevance methods", aim at evaluating the impact of each input feature on the predictions. These methods have originally been used to explain network predictions, but have also recently been used to constrain the learning of these models. These models either use occlusion-based or gradient-based attribution methods.\par
Occlusion-based methods \cite{zeilerocclusion} evaluate the attribution of a certain patch of pixels by comparing the predictions given by the input image with the predictions given by the occluded input image.
For instance, Du \textit{et al.} \cite{du2019learning} applied this to a Natural Language Processing (NLP) problem and proposed to sparsify the explanations by reducing the score of non-important features using expert-annotated important clauses in the input sentences. 'Negative examples' are created by removing these clauses from the input sentences. However, computing occlusion-based attributions can have a very high computational cost especially on image data.\par
% These methods tend to be very slow and very much depend on the number of input features that are evaluated.\par
To reduce the evaluation time of these methods, gradient-based attribution methods were introduced. Simonyan \textit{et al.} \cite{simonyan2014deep} first introduced image-specific class saliency maps. Selvaraju \textit{et al.} \cite{grad_cam}, with \textit{Grad-CAM}, created a class-specific attribution method to produce visual explanations, and also used it for weakly-supervised segmentation \cite{grad_cam}. Grad-CAM computes heatmaps by multiplying each channel of the last convolutional feature map by its "importance" (the mean over that specific channel of the gradient of the chosen output class w.r.t. the last convolutional layer's output). In 2016, Shrikumar \textit{et al.} \cite{shrikumar2017just} proposed a technique to sharpen the attribution maps called \textit{Gradient*Input}, where the partial derivatives of the output are multiplied by the input features. The idea is that the gradient tells us how important a certain feature is, and the input tells us how strongly it is expressed in the final prediction. Other propagation-based methods have been introduced in the second half of the 2010's like \textit{Integrated Gradients} (Sundarajan \textit{et al.} \cite{sundararajan2017axiomatic}), which is more stable than \textit{Gradient*Input} and satisfies the completeness axiom, which generally better captures the explanation of each input feature, at the cost of a larger computational load. \par
% \textit{Layer-wise Relevance Propagation} (Bach \textit{et al.} \cite{Bach2015OnPE}) and \textit{DeepLIFT} (Shrikumar \textit{et al.} \cite{pmlr-v70-shrikumar17a}) proceed in a backward fashion and redistribute the relevance score layer by layer, however \textit{DeepLIFT} computes the relevance score of an input feature compared to a reference input (often zero). Comparisons of these methods' correlations (Ancona \textit{et al.} \cite{ancona2018better}) as well as analyses of the properties of these methods have also become important recently.\par
% Attribution maps can also be constrained during training to obtain better explanations or to improve the predictive power of a model, as we will see in the next section.

% \subsubsection{Constrained Attribution Learning}

% Attribution methods have been used to explain network predictions, but have also recently been used to constrain the learning of these models. These models either use occlusion-based or gradient-based attribution methods.\par
% On the one hand, some methods decide to constrain occlusion-based attribution methods. For instance, Du \textit{et al.} \cite{du2019learning} applied this to a Natural Language Processing (NLP) problem and proposed to sparsify the explanations by reducing the score of non-important features using expert-annotated important clauses in the input sentences. 'Negative examples' are created by removing these clauses from the input sentences. However, computing occlusion-based attributions can have a very high computational cost especially on image data.\par
For efficiency reasons, some models decide to constrain gradient-based attributions. However, there are different ways to constrain this attribution. Erion \textit{et al.} \cite{erion2020improving} decided to constrain their model so that its attributions would satisfy desirable properties. They therefore introduced an attribution method called 'Expected Gradients', which guarantees that the attributions don't depend on the method's implementation \cite{ancona2018better}. They use 'Expected Gradients' to improve their predictive capacity by constraining it to have more desirable properties like sparsity and smoothness. Nevertheless, they don't make use of extra information which could help them in identifying key features.\par
Attribution methods can also be guided by the use of privileged information. Liu \textit{et al.} \cite{liu2019incorporating} applied this to NLP and added a constraining term to their loss with a L2 norm between their attribution (Integrated Gradients) and their prior information (toxic or non-toxic words). In 2017, Ross \textit{et al.} \cite{ross2017right} introduced the idea of being "right for the right reasons" (RRR) for Computer Vision. They regularize the gradients of the input features w.r.t. the outputs by penalizing the 'unimportant' features with a prior binary mask. This mask indicates whether or not a certain feature should be relevant for a certain prediction. However, in their paper, they only constrain their gradient inputs to improve their explanations, and not to improve the performance of their model.\par
% The methods presented in this section constrain their attributions to improve their explanations. 
On the contrary, we use the attribution maps to spatially constrain the learning process in order to improve the predictive power of a FER model. Therefore, we will present spatially constrained methods for Facial Expression tasks. 
% Constraining the learning process of a model can be used on Facial Expression tasks, as will be presented in the next section. 

\subsubsection{Constrained Learning for Facial Expression tasks}

Spatially constrained methods have become very popular in various Facial Expression tasks because of the importance of certain areas of the input images, for example eyes, eyebrows or the mouth.\par
First of all, some methods learn to guide their model with specific spatial modules. This way, Zhao \textit{et al.} with EfficientFace \cite{efficient} used an approach in which the model learns to dynamically focus on local and global salient facial features with a local-feature extractor. This method learns the important spatial features without a semantic prior, and therefore doesn't guarantee that it is focusing on the important areas. This can also be a problem for its explainability.\par
Second, some methods use semantic information learnt from intermediary tasks to improve their predictions on their main task. Shao \textit{et al.} \cite{jaanet} proposed JAA-Net, which aims to predict Facial Action Units by learning to predict face alignment points first. They then use the face alignment features to refine attention maps that guide the Facial Action Unit detection. This method leverages a prediction relative to another task to spatially guide its model on the main task. Pu \textit{et al.} \cite{pu2021auexpression} have proposed a FER method that constrains the model by predicting facial action units first. These methods need explicit predictions for an intermediary task for their model to focus on the important areas. \textbf{These methods strongly depend on the efficiency of their model on the intermediary task. This way, the process is more complex and makes the predictions on the main task more error-prone}.\par
Another way of guaranteeing that the model focuses on the most salient areas can be to directly take advantage of additional information. For example, Jacob \textit{et al.} \cite{Jacob_2021_CVPR} used heatmaps, where the areas of the facial action units are highlighted, as prior information for Facial Action Units prediction. In this method, they build attention maps and constrain them to resemble the prior information attention maps. This allows the model to focus on specific areas that are key to predict the presence of an action unit. The said method uses a semantic prior at training time to guide its model towards specific important areas, without needing it to predict at test time. \textbf{However, they only constrain attention maps created by a separate network branch, which doesn't directly guarantee that the model focuses on these salient areas. On the contrary, PAL leverages additional semantic information in a more straightforward way by guiding its attribution maps, and therefore the exact areas that the model concentrates on.} Furthermore, our method offers to improve the model's predictive power by forcing the attributions to concentrate on certain areas while still leaving them a certain degree of liberty.\par
In the next section, we will present our methodology, first focusing on the different possible attribution methods, then our loss and channel strategy. Finally, we will explain our heatmap prior information.\par

==> sections/response.tex <==

\renewcommand{\baselinestretch}{1.0} 

\newcommand{\kevin}[1]{{\color{red}#1}}

\newcommand{\arnaud}[1]{{\color{blue}#1}}

\definecolor{dg)}{rgb}{0.0, 0.5, 0.0}
\newcommand{\jules}[1]{{\color{green}#1}}
\pagebreak
{\bfseries\LARGE General Response:\par}
\medskip
We would like to thank the reviewers for their interest in the proposed method and their constructive commentary that will enable us to improve the quality of the paper. All reviewers gave positive feedback concerning the interest and novelty of the method. However, they have also pointed out areas for improvement, which we now address individually for each reviewer.\medskip

{\bfseries\LARGE Reviewer 1:\par}
\medskip
\textbf{1- Elaborate in more detail on the problems encountered in the study of FER and how the proposed method is targeted to solve this issue:} The problem of FER is difficult because the datasets at hand are rather small (compared to e.g. Imagenet) but however encompass a number of factors of variations (e.g. different morphological traits, non-frontal head poses, and so on). As a result, the networks have a hard time selecting relevant information in order to learn proper expression classification.

%\kevin{(compared to e.g. imagenet for object recognition) and because of noisy data (perceived emotions bears some degree of subjectivity thus their interpretation may vary depending on the annotator). From a learning perspective, this can makes things harder for a network to find out where the relevant information is in the image}. 

The proposed method alleviates these problems by guiding the network to concentrate on crucial areas of the input image. This allows for CNN-based models to reach high performance levels without the need for extremely large datasets. This is discussed in lines 4-13 of the Introduction of the revised manuscript.
\medskip
\par
{\bfseries\LARGE Reviewer 2:\par}
\medskip
\textbf{1- There is no direct mention of transformers in Section 2: Related Works:}     %Thank you for pointing this out. We indeed talk about Transformers in the second paragraph of II.1) without explicitly using the word "Transformer".\newline
%Transformers have originally been introduced by Vaswani \textit{et al.} \cite{transformers} and widely used for NLP. These models have since been used for Computer Vision (ViT by Dosovitskiy \textit{et al.} \cite{1616} for example).
% These models divide their input images into several patches and provide embeddings of these patches using a Transformer decoder.\newline
%These models use the concept of "cross-attention" where they compute an attention matrix between patches of the image and the different classes. This allows the model to understand which areas of the image are more important to predict a certain class. In our paper, we decide to guide the "attribution" of our model, which corresponds to the relevance of an input feature (or intermediate feature) on the output to understand what pixels are important for our predictions. The fact that we work with gradient-based attribution methods to understand what pixels are important for our predictions whereas classical image Tranformers use "cross-attention" to find which patches are more important in the prediction of each class constitutes a first difference between Transformers and our method. \newline
%Secondly, we decide to guide our model towards salient facial features by constraining its attribution maps to resemble facial landmark heatmaps, whereas classical Transformers such as ViT learn which areas of the input images are more important for the prediction of a certain class without the help of any additional information.
% In this sense, these models learn to focus on the most important patches of the input images. On the opposite, our method guides the model's attribution using additional information.\newline
%We changed the second paragraph of II.1) to introduce transformers and make our position towards them clearer.

We believe that refering to \textit{attention} in the paper was misleading and changed in to \textit{attribution} everywhere: for instance, in the context of transformer architecture, \textit{attention} refers to a multiplicative mechanism that is used to select the most relevant parts of an input based on another (\textit{cross-attention}) or the same input (\textit{self-attention}). It is embedded within the network architecture during training and used at inference time. Conversely, our method constrains, during the training phase, the \textit{attribution} maps (the derivatives of the network output w.r.t. its input) to match a specific spatial prior (a map derived from facial landmaks) : in other words, we encourage the network to focus on specific face areas at train time and, at inference time, the network has learnt to do so, henceforth not requiring this external (privileged) information anymore.

Thus, the \textit{attention} mechanism used in transformers and the proposed constrained \textit{attribution} method based on privileged information are two very distinct mechanisms. To avoid any confusion, we removed any reference to the term attention (in the machine learning sense) in the paper.

Nevertheless, we agree that transformers are an important trend in computer vision in general and in expression recognition in particular : therefore, we added the proposed references, and discussed them in the related work Section to highlight the difference with the proposed method.


\par
\textbf{2- Experiments in IV.E.1 are not very informative. While extensive results are always appreciated and the results are perfectly acceptable, it would be preferable to use additional space for more informative results:}     %These experiments are used to explain the results observed in the RAF-DB confusion matrix. The revised version of the paper allows for 2 extra pages, and we therefore choose to leave this subsection in the paper because we can still answer comments 3- and 4- from Reviewer 2. \kevin{il me semble qu'il disait aussi que ce n'était pas inintéressant mais pas le plus important, on pourrait peut-être laisser cette partie là de la quetion}\par

We added the suggested experiments to the revised paper (see response to comments 3 and 4).

\textbf{3- There is no discussion or experiment on the impact of given facial landmarks on en performance of the model:}     

% \begin{figure}
% \centering
% \includegraphics[width=88mm]{images/sensi_landmarks.png}
% \caption{Performance of the model learnt with heatmaps created with noisy landmarks (evaluation for different values of sigma).}
% \label{fig:sensi_landmarks}
% \end{figure}

% \begin{figure*}[!t]
% \centering
% \subfloat{\includegraphics[width=0.825in]{images/noisy_heatmaps/test_0001_aligned1.png}%
% \label{sigma1}}
% \hfil
% \subfloat{\includegraphics[width=0.825in]{images/noisy_heatmaps/test_0001_aligned2.png}%
% \label{sigma2}}
% \hfil
% \subfloat{\includegraphics[width=0.825in]{images/noisy_heatmaps/test_0001_aligned3.png}%
% \label{sigma3}}
% \hfil
% \subfloat{\includegraphics[width=0.825in]{images/noisy_heatmaps/test_0001_aligned4.png}%
% \label{sigma4}}
% \hfil
% \subfloat{\includegraphics[width=0.825in]{images/noisy_heatmaps/test_0001_aligned5.png}%
% \label{sigma5}}
% \caption{Examples}
% \label{noisy_heatmaps}
% \end{figure*}

We conducted an experiment to evaluate the sensitivity of the method to the correctness of the privileged information. To do this, we learnt a VGG-based model using PAL with noisy heatmaps. We created heatmaps derived from landmarks that were sampled from a gaussian distribution centered in the correct landmark's value with a sigma whose value varied between 2 and 5. The results and the analysis are reported on the revised paper in section IV.C.4.

% created heatmaps derived from noisy landmarks (we sampled from a gaussian distribution with sigma equal to 2, 3, 4 and 5). Examples of these heatmaps can be found in Figure \ref{noisy_heatmaps}. We can observe from Figure \ref{fig:sensi_landmarks} that the model learnt with the correct heatmaps (sigma=0) performs better than with the incorrect heatmaps. Even though the mean accuracy score of this method decreases while the value of sigma increases, we see that the model performs better than the baseline, which can be explained by the fact that the heatmaps still highlight interesting areas of the face. Furthermore, this shows that the method is robust to certain inaccuracies in the prior information.  }
\par
\textbf{4- It would be interesting to evaluate different values of C1 (equation 7):}    This is an interesting question to understand the balance between guiding the model and leaving some freedom for it to concentrate on different parts of the image. We conducted experiments for several values of $C_1\in\{C/4, C/2, 3C/4, C\}$. These experiments have been reported on the revised version of the paper on Table II and discussed in IV.C.3).\newline
Results show that guiding the mean of $3/4$ of the channels obtains similar scores in accuracy as using the \textit{Mean} channel strategy ($86.32$ for $C_1=3C/4$ and $86.38$ for $C_1=C$). However, when guiding the mean of $1/4$ of the channels, we obtain a mean accuracy score of $86.55$, which outperforms the baseline accuracy by \text{1.55\%}.
% \jules{, but with a more important standard deviation, which we could explain by the further freedom given to the model, whose unconstrained channels could learn to concentrate on more or less important features.} \kevin{(avec cette explication, le VGG sans pal devrait avoir une variance encore plus grande, non ?)}.
The best mean accuracy results are still obtained when taking $C_1=C/2$ (\textit{Mean of Half} strategy), which shows that while guiding the majority of our model still works better than learning a simple CNN without any privileged information, leaving the model more freedom to concentrate on different areas of the picture helps it generalize better.\par
% We can also observe in Figure 6 of the revised paper that the channels that aren't directly constrained by PAL mainly concentrate on one or some of the crucial facial features (mostly the mouth for image 5 for example), which shows that the attention \kevin{éviter ce terme ?}\arnaud{intérêt de cette phrase? Je ne comprends pas où tu veux en venir exactement} is an important source of information for the model.  \par
\textbf{5- Table II does not contain standard deviations:}      
% In Table II, we compare our method's results with the state-of-the-art's best results on RAF-DB and AffectNet. In the papers to which we compare our results, standard deviations are not reported either. \jules{An analysis of the variance is discussed in Figure 3 and Table 2 of the revised paper. Also, PAENet \cite{PAENet}, the runner-up on AffectNet, predicts three tasks jointly using lifelong learning, and therefore learns to predict emotion with additional tasks and datasets. FDLR \cite{fdlr}, the runner-up on RAF-DB, uses 4 separate modules added to their ResNet-based backbone. Seeing as RAF-DB has only 12K images, and the AffecNet reports an annotator's agreement of only 60.7\%, we believe that a small improvement on both datasets is generally convincing.}\kevin{ok toutes les infos sont là mais il faut mieux structurer le discours, par ex. : 1. on a fait une étude de variance avant dans le papier, 2. on ne l'a pas reporté dans la comparainon avec le sota car on n'a pas l'info pour ces méthodes et du coup l'intérêt est limité, 3. ton discours sur les perfs et le nombre d'image, 4. autres avantages de notre méthode par rapport au sota (nombre de paramètres, base de données supp., ...} \par

An analysis of the variance of the results is discussed in Figure 3 and Table 2 of the revised paper. In Table II, we compare our method's results with the state-of-the-art's best results on RAF-DB and AffectNet. In the papers to which we compare our results, standard deviations are not reported either and we believe they are therefore not very relevant. Seeing as RAF-DB has only 12K images, and the AffecNet reports an annotator's agreement of only 60.7\%, we believe that a small improvement on both datasets is generally convincing. Finally, PAENet \cite{PAENet}, the runner-up on AffectNet, predicts three tasks jointly using lifelong learning, and therefore learns to predict emotion with additional tasks and datasets. FDLR \cite{fdlr}, the runner-up on RAF-DB, uses 4 separate modules added to their ResNet-based backbone.\par
\textbf{Writing - 1- do not agree with the choice of "Privileged" as a way to refer to the attention-based mechanism: }     
% Our method uses additional information (also called "Privileged Information") during training to focus on certain areas of the input image, but doesn't need these at inference time. The notion of "Learning under Privileged Information" (LUPI) was introduced by Vapnik and Vashist \cite{lupi} \kevin{partie pas necessaire: where they compare machine learning to human learning. In this sense, adding additional information $x^*$ to sample $x$ can be compared to the explanations or comments that a teacher adds on top of their examples.} While \cite{lupi} uses Privileged Information to extend the works on support vector machines, several other works have explored LUPI for different tasks and architectures: Hoffmann \textit{et al.} \cite{darrell} use depth images as privileged information added to RGB images to improve their model's scores for object detection, and Lambert \textit{et al.} \cite{Lambert2018DeepLU} introduce a new LUPI paradigm for CNNs and RNNs, and tested it on image classification and machine translation.\par
% We therefore believe that the use of the word "Privileged" in the paper is correct, \kevin{as it is closely related to the one that is commonly used by the community in this context.} \arnaud{C'est trop long, tu dis en 10 lignes un truc qui peut être résumé en 3. Par ailleurs tu noies tellement le poisson qu'on en oublie l'essentiel: privileged information=info disponible seulement au moment du train, pas du test. citer 2 3 articles, conclure que l'utilisation est ok}\par
The notion of "Learning under Privileged Information" (LUPI) was introduced by Vapnik and Vashist \cite{lupi} where they compare machine learning to human learning. In this sense, adding supplementary information $x^*$ to sample $x$ can be compared to the explanations or comments that a teacher adds on top of their examples. In practice, LUPI means that the model guides the learning using additional information only available during training, and not during inference. Other papers like \cite{darrell} (Hoffman \textit{et al.}) and \cite{Lambert2018DeepLU} (Lambert \textit{et al.}) extended these works to tasks such as object detection and to architectures such as CNNs and RNNs.\par
Our method uses additional information (heatmaps of facial landmarks) during training to focus on certain areas of the input image, but doesn't need these at inference time. We therefore believe that the use of the word "Privileged" in the paper is correct, as it is closely related to the one that is commonly used by the community in this context.\par
\textbf{Writing - 2- do not understand Equation 8 as it is written} Thank you for your feedback. Looking back, the equation wasn't very clear indeed and we changed it to the proposed writing (see changes in III.D.)\par
\textbf{Writing - 3-} The typos have been corrected in the revised version.\par
\medskip
\par
{\bfseries\LARGE Reviewer 3:\par}
\medskip
\textbf{1- The core contribution of this paper seems to be a privileged attribution LOSS:}  
% \textit{est-ce qu'on change le titre pour Privileged Attribution Loss for FER ?? c'est pas faux mais les réseaux sont quand meme constrained et on ne peut pas changer la loss} \kevin{on a dit hier qu'on ne changeait pas le titre, il faut jute trouver les mots pour le dire. }\par
Although we agree with the reviewer's comment that PAL is indeed the core contribution of this paper, our method explicitly constrains the attribution maps of a Deep Neural Network with privileged information. Therefore, we believe that the title of the paper is still a fitting choice.\par
\textbf{2- The results shown in Table 2 are only slightly better than state-of-the-art results:}   We improve state-of-the-art results on both RAF-DB and AffectNet which are very competitive datasets. This demonstrates the effectiveness of our method. Furthermore, our method is very simple and doesn't need additional information at inference time, where it only needs to run a simple CNN. Conversely, as it is discussed in the response to the second point of Reviewer 2, PAENet \cite{PAENet}, the runner-up on AffectNet, predicts three tasks jointly using lifelong learning, and therefore learns to predict emotion with additional tasks and datasets. Also, FDLR \cite{fdlr}, the runner-up on RAF-DB, uses 4 separate modules added to their ResNet-based backbone.\par
\textbf{3- The authors should provide the confusion matrix on the AffectNet database:}      The confusion matrix for the AffectNet test set has been added to the revised version of the paper. It is Figure 6.


==> tables/ablation_table.tex <==
\begin{table}[!t]
% increase table row spacing, adjust to taste
    \renewcommand{\arraystretch}{1.1}
    % if using array.sty, it might be a good idea to tweak the value of
    % \extrarowheight as needed to properly center the text within the cells
% Some packages, such as MDW tools, offer better commands for making tables
% than the plain LaTeX2e tabular which is used here.
	\caption{Ablation study on RAF-DB dataset comparing different attribution methods and channel strategies.}
	\label{ablation}
	\centering
	\resizebox{8.5cm}{!}{
    \begin{tabular}{|c||c|c|c|c|c||c||c|}
    \hline
    \textbf{Method} & $Attribution$ & $Channels$ & $Acc$ \\
    \hline
    $VGG16 $ & $---$ & $---$ & $85.17$ \\
    \hline
    $VGG16  + PAL$ & $Grad$ & All Channels & $85.59$ \\
    $VGG16  + PAL$ & $Grad$ & Mean & $86.34$ \\
    $VGG16  + PAL$ & $Grad$ & Mean of half & $ 86.47 $\\
    $VGG16  + PAL$ & $Grad*Input$ & Mean & $86.64$ \\
    $VGG16  + PAL$ & $Grad*Input$ & Mean of half & $86.86$ \\
    
    \hline
    \end{tabular}
    }
\end{table}

==> tables/affectnet_results.tex <==
\resizebox{6cm}{!}{
    \begin{tabular}{|c||c|}
    \hline
    \textbf{Method} & Accuracy\\
    \hline
    Baseline & 62.14 (a refaire) \\
    \hline
    % THIN \cite{thin} & 63.97 \\
    DACL \cite{Farzaneh_2021_WACV} & 65.20 \\
    PAENet \cite{PAENet} & 65.29 \\
    Distilled Student \cite{distilled} & 65.40 \\
    % TransFER \cite{xue2021transfer} & \textbf{66.23} \\
    \hline
    Ours (Resnet50) & 65.83\\
    \hline
    \end{tabular}
    }

==> tables/old_result_table.tex <==
\resizebox{6cm}{!}{
    \begin{tabular}{|c||c|c|}
    \hline
    \textbf{Method} & RAF-DB & AffectNet\\
    \hline
    gACNN \cite{gacnn} & 85.07 & 58.78 \\
    IPA2LT \cite{Zeng_2018_ECCV} & 86.77 & 57.31 \\
    % DDA Loss \cite{Farzaneh2020DiscriminantDL} & 86.9 & 62.34 \\
    THIN \cite{THIN} & 87.81 & 63.97 \\
    DACL \cite{Farzaneh_2021_WACV} & 87.78 & 65.20 \\
    EfficientFace \cite{zhao2021robust} & 88.36 & 63.70 \\
    PSR \cite{psr} & 88.98 & 63.77\\
    PAENet \cite{PAENet} & -- & 65.29 \\
    Distilled Student \cite{distilled} & -- & 65.40 \\
    DMUE \cite{DMUE} & 89.42 & --\\
    FDLR \cite{fdlr} & 89.47 & --\\
    % TransFER \cite{xue2021transfer} & \textbf{90.91} \\
    \hline
    Baseline (Resnet50) & 88.6 & 62.14\\
    \hline
    Ours (Resnet50 + PAL) & \textbf{89.54} & \textbf{65.83} \\
    \hline
    \end{tabular}
    }

==> tables/raf_results.tex <==
\resizebox{6cm}{!}{
    \begin{tabular}{|c||c|}
    \hline
    \textbf{Method} & Accuracy\\
    \hline
    Baseline & 88.6 (a refaire)\\
    \hline
    PSR \cite{psr} & 88.98 \\
    DMUE \cite{DMUE} & 89.42 \\
    FDLR \cite{fdlr} & 89.47 \\
    % TransFER \cite{xue2021transfer} & \textbf{90.91} \\
    \hline
    Ours (Resnet50) & 89.54\\
    \hline
    \end{tabular}
    }

==> tables/rafdb_table.tex <==
\resizebox{9.2cm}{!}{
    \begin{tabular}{|c||c||c||c||c||c||c||c|}
    \hline
    \textbf{Class} & surprise & fear & disgust & happiness & sadness & anger & neutral \\
    \hline
    Train & 1290 & 281 & 717 & 4772 & 1982 & 705 & 2524 \\
    \hline
    Test & 329 & 74 & 160 & 1185 & 478 & 162 & 680 \\
    \hline
    \end{tabular}
    }

